MEGAN: A Generative Adversarial Network for Multi-View Network Embedding

Data from many real-world applications can be naturally represented by multi-view networks where the different views encode different types of relationships (e.g., friendship, shared interests in music, etc.) between real-world individuals or entities. There is an urgent need for methods to obtain low-dimensional, information preserving and typically nonlinear embeddings of such multi-view networks. However, most of the work on multi-view learning focuses on data that lack a network structure, and most of the work on network embeddings has focused primarily on single-view networks. Against this background, we consider the multi-view network representation learning problem, i.e., the problem of constructing low-dimensional information preserving embeddings of multi-view networks. Specifically, we investigate a novel Generative Adversarial Network (GAN) framework for Multi-View Network Embedding, namely MEGAN, aimed at preserving the information from the individual network views, while accounting for connectivity across (and hence complementarity of and correlations between) different views. The results of our experiments on two real-world multi-view data sets show that the embeddings obtained using MEGAN outperform the state-of-the-art methods on node classification, link prediction and visualization tasks.

==> 2amversion.tex <==
\section{Multi-View Network Embedding GAN}
In what follows, we define the multi-view network embedding (MVNE) problem before proceeding to describe the key components of MVNE-GAN, our proposed solution to MVNE.
\subsection{Multi-View Network Embedding}
A multi-view network is defined as $\mathcal{G} = (\mathcal{V} ,\mathcal{E})$, where $\mathcal{V}= \{v_1, v_2, \dots, v_n \}$ denotes the set of nodes and $\mathcal{E}=\{\mathcal{E}^{(1)},\mathcal{E}^{(2)}, \dots, \mathcal{E}^{(k)}\} $ describes the edge sets that encode  $k$ different relation types (views).
For a given relation type $l$, $\mathcal{E}^{(l)} = \{e_{ij}^{(l)}\}_{i,j=1}^n$ specifies the presence of the corresponding relation between node $v_i$ and node $v_j$. Thus, $e_{ij}^{(l)}=1$ indicates that $v_i$ and $v_j$ has a link for relation $l$ and 0 otherwise.  We use $\mathcal{K}_{ij} = (e_{ij}^{(1)}, \dots, e_{ij}^{(k)})$ to denote the connectivity of $(v_i,v_j)$. The goal of multi-view network representation learning is to learn $\mathbf{X} \in \mathbb{R}^{n \times d}$, a low-dimensional embedding of $\mathcal{G}$, where $d \ll n$ is the latent dimension.

\begin{figure}[ht!]
      \centering
   %   \vskip -1em
        \includegraphics[width=8.6cm]{archframe2.pdf}
 %       \vskip -1em
        \caption{The architecture of the  MVNE-GAN framework. The pair of of orange nodes, e.g., $(v_1,v_2)$,  denote {\em positive} link in the sampled data, and $(v_1,v_4)$ denotes a {\em negative} node pair sampled from the generative model $p_g$. The parameters in generator are updated with gradient descent using a variant of the standard minimax objective function for GAN.}
        \label{fig:model_architecture}
\end{figure}
%type of each relation $e^{(l)} = \{ e_{ij}^{(l)}\}_{i,j=1}^{|l|}$, . 

%between node set $\Phi^{(k)} (\mathcal{V})$. For type of each relation $e^{(l)} = \{ e_{ij}^{(l)}\}_{i,j=1}^{|l|}$, 


\subsection{\textbf{Multi-view Generative Adversarial Network}}
Figure~\ref{fig:model_architecture} illustrates the architecture of MVNE-GAN. MVNE-GAN consists of two modules, a generator $G(\mathcal K_{ij})$ and a discriminator $D$. Unlike a GAN designed to perform single-view network embedding, which needs  to model only the connectivity among nodes within a single view, the generator $G$ of MVNE-GAN needs to capture the multi-view network topology which is the connectivity among nodes within each view as well as the correlations between views. Given a pair of nodes $(v_i, v_j)$, $G$ takes the embeddings of $v_i$ and $v_j$ to generate the probability of $v_i$ and $v_j$ are connected in each view. For the pair of nodes sampled from real-world multi-view network, e.g., $(v_1, v_2) \sim p_{data}$ in Figure~\ref{fig:model_architecture}, the generator can produce (or choose) a \textit{fake} node $v_4$ with the connectivity pattern between $v_1$ and $v_4$ being sufficiently similar to that of the sampled pair of node to fool the discriminator. The discriminator $D$ is trained to differentiate if a pair of nodes input to it is \text{real} or \textit{fake}. With the minmax game between $D$ and $G$, we will show that upon convergence, we are able to learn embeddings that $G$ can use to generate the multi-view network. In other words, the embeddings capture the connectivity among nodes within each views and the correlations between views. Next, we introduce the details of $G$, $D$ and an efficient sampling strategy.

\subsubsection{Multi-view Generator}
Recall that goals of multi-view generator $G$ are to \textbf{(i)} generate the multi-view connectivity of adversarial nodes that
fools the discriminator D; and \textbf{(ii)} learn an embedding  that captures the multi-view network topology. To ensure that it achieves the goals, we design the multi-view generator consisting of two components: one fusing generator $G_f$ and $k$ connectivity generators $G^{(l)}$. Let $\mathbf{X} \in \mathbb{R}^{n \times d}$ be the embedding matrix, then the representation of $v_i$ can be obtained as $\mathbf{e}_i \mathbf{X}$, where $\mathbf{e}_i$ is the one-hot representation with $i$-th value as 1. The fusing generator $G_f$ firstly fuses the representation of $v_i$ and $v_j$, aiming to capture the correlation between $v_i$ and $v_j$.  We use $G_f(v_i, v_j; \mathbf{X}, \theta_f)$ to denote the fused representation where $\theta_f$ is its parameters. Then, the fused representation is then used to calculate the probability of $e_{ij}^{l}=1$ for $l=1,\dots, k$. This can be formally written as:
\begin{equation}
\small
\begin{split}
G(e^{(1)}_{ij},\dots,e^{(k)}_{ij}|v_i,v_j,\theta_G)= \prod_{l=1}^kG^{(l)}(e^{(l)}_{ij}|G_f(v_i,v_j;\mathbf{X},\theta_c);\theta^{(l)})
\end{split}
\label{eq4:g}
\end{equation}
%In Eq.(\ref{eq:DisImp}), 
%$\theta = \{\theta_c, \theta^{(1)}, \dots, \theta^{(k)}\}$ 
where $G^{(l)}$ is the connectivity generator for generating the connectivity in between $(v_i,v_j)$ in view $l$ given the fused representation. $\theta_G=\{\mathbf{X}, \theta_f, \theta^{(l), l =1, \dots, k}\}$ is the parameter for the multi-view generator $G$. Because each $G^{(l)}$ of $k$ generators are independent given the fused representation, the corresponding parameter $\theta^{(l)}$ can be optimized independently in parallel. We use two layer multi-layer perceptron (MLP) to implement $G_f$ and each $G^{(l)}$. Actually, more complex deep neural networks could replace the generative model outlined here. We leave exploring feasible deep neural networks as a possible future direction.

\subsubsection{Node Pair Discriminator}
The goal of $D$ is to discriminate between the positive node pairs from the multi-view network data and the negative node pairs produced by the generator $G$ so as to enforce $G$ to more accurately fit the distribution of multi-view network connectivity. For this purpose, for an arbitrary node pair sampled from real-data, i.e., $(v_i,v_j) \sim p_{data}$, $D$ should output 1, meaning that the sampled wwnode pair is real. To fool the discriminator, for each $(v_i,v_j) \sim p_{data}$, we propose to sample a pair of negative nodes from $G$ that has connectivity that is similar to that of  $(v_i, v_j)$, e.g., $(v_i, v_c) \sim p_G$ with $\tilde{\mathcal{K}}_{ic}=\mathcal{K}_{jc}$, where $p_G$ denotes the distribution modeled by $G$. In particular, we choose the one that has the highest probability, i.e.,
\begin{equation}
    \argmin_{v_j \in \mathcal V}\prod_{l=1}^k p(e^{( m)}_{ic}|v_j,v_c)
    \label{eq:select}
\end{equation}
The intuitive motivation behind the sampling strategy in Eq.(\ref{eq:select}) is that the negative node pair $(v_i, v_c)$ is more likely to fool the connectivity discriminator if connectivity $\tilde{\mathcal{K}}_{ic}$ is the same to the connectivity $\mathcal{K}_{ij}$ of the positive pair $(v_i, v_j)$. 
% The reason we want to select the node $v_j$ that has the highest probability of having $\mathcal{K}_{jc}=\mathcal{K}_{ic}$ is because we want to fool the discriminator. The one that has the highest probability of having the same connectivity is more likely to fool the discriminator. 
Given such a negative or fake edge (pair of nodes), the discriminator should output 0, whereas $G$ should aim to assign high enough probability to negative edges that can fool $D$. 
As  $D$ learns to distinguish the negative edges from the positive ones, the $G$ captures the connectivity distribution of the multi-view graph. 
%With such minmax game, for a given pair of nodes $(v_i, v_c)$, when we want to sample $(v_j, v_c)$ with $\tilde{\mathcal{K}}_{ic}=\mathcal{K}_{jc}$, we can expect the generator will gradually assign higher probability to $(v_i, v_c)$ because this is the one that can finally fool the discriminator upon convergence. 
We will show this in Section~\ref{sec:theorectical_analysis}.
%For any $(v_i, v_j)\simp_{data}$ and $(v_i, v_a)\simp_{g}$ 
%\begin{equation}
%    p(1|v_i,v_j)p(0|v_i,v_a)
%\end{equation}
%In other words, the discriminator $D(v_i, v_j; \theta_D)$ needs to discriminate the label $y_{ij}$ (either positive represented by $1$ or negative represented by $0$) for the given training vertex pair $(v_i,v_j)$. 

We define the $D$ as the sigmoid function of the inner product of the input node pair $(v_i,v_j)$:
\begin{equation}
\small
   D(v_i,v_j) =  \frac{\exp(\mathbf{d_i}^T\cdot \mathbf{d_j})}{1+\exp(\mathbf{d_i}^T\cdot \mathbf{d_j})}
   \label{eq2:d}
\end{equation}
where $\mathbf{d}_i$ and $\mathbf{d}_j$ denote the $d$ dimensional representation of node pair $(v_i,v_j)$. It is worth noting that $D(v_i,v_j)$ could be any differentiable function with domain $[0,1]$. We choose the sigmoid function for its stable property and leave the selections of $D(\cdot)$ as a possible future direction.

\subsubsection{Efficient Negative Node Sampling}
In Practice, for one pair of nodes $(v_i,v_j)$, in order to sample a pair of nodes $(v_i, v_c)$ from $G$, we need to calculate $\prod_{l=1}^kp(e^{(l)}_{ic}|v_j,v_c)$ for all $v_j \in \mathcal{V}$ and select the one with the highest probability, which can be very time-consuming. To make the sampling more efficient, instead of calculating the probability for all nodes, we  calculate the probability  for neighbors of $v_c$, i.e., $\mathcal{N}(v_c)$, where $\mathcal{N}_{v_c}$ is the set of nodes that have connectivity to $v_c$ for at least one view in real network. In other words, we only sample from $\mathcal{N}(v_c)$. The size of $\mathcal{N}(v_c)$ is significantly smaller than $n$ because the network is usually very sparse, which makes the sampling very efficient. Thus, we would expect that for positive sample $(v_i,v_c) \sim p_G$, any negative sample $(v_j,v_c)$ should have a node $v_j$ from $v_c$'s neighbor.  


%{\color{blue} to revise} In multi-view graph scenario, one key question is how to draw positive and negative samples in the training phase efficiently. One kind of typical sampling strategies in graph representation learning is to collect random walks sequences via treating nodes as words from the language modelling perspective. In the multi-view graph cases, however, such strategy could not diffuse among views since there are no cross-view links. Another kind of typical sampling strategies is to sample the neighbors vertices randomly from its neighbors since the transit probability is equal to the connectivity distribution. Such method could not be directly extended to multi-view graph scenarios due the connectivity distribution could not be approximate by the transit probability.

% In the paper, we propose the sampling strategy to sample the positive vertices pair and its corresponding negative vertices pair from the multi-view network efficiently. During training process of MVGAN, we firstly sample the positive vertices pair $(v_i,v_j)$ over vertices set $\mathcal V$ randomly with the multi-view connectivity information $\mathcal{K}_{ij}$. Then for the given vertex $v_i$, we select $v_a$ from the $\mathcal V$ as:
% \begin{equation}
%     \argmin_{v_a \in \mathcal V}\prod_{l=1}^kp(e^{(l)}_{ij}|v_i,v_a)
%     \label{eq:select}
% \end{equation}




\subsubsection{Objective Function of MVNE-GAN}

% In multi-view network, we assume that the connectivity information $\mathcal{K}_{ij} = (e_{ij}^{(1)}, \dots, e_{ij}^{(k)})$ of the vertex pair $(v_i,v_j)$ reveals the connectivity distribution $p_{data}(\mathcal{K}_{ij}|v_i,v_j)$. %among $k$ types of relations. 
% In the MVGAN model, we propose a connectivity generator $G$ which tries to capture the connectivity distribution  $p_{data}(\mathcal{K}_{ij}|v_i,v_j)$ of pair $(v_i,v_j)$ and generate the negative vertex pair $(v_i,v_a)$ to fool the connectivity discriminator $D$. Meanwhile, we train the connectivity discriminator $D$ which learns to distinguish the positive vertices pair sampled from $p_{data}(\mathcal{K}_{ij}|v_i,v_j)$ and the adversarial vertices sampled from $p_g(\tilde{\mathcal{K}}_{ia}|v_i,v_a)$. The joint value function $V(G,D)$ could be define as:
With the generator $G$ modeling the multi-view connectivity so as to generate adversarial samples that could fool the discriminator, the discriminator to differentiate between true edges (pairs of nodes) from fake edges as well as an efficient negative sampling strategy, we can specify the objective function for MVNE-GAN: 
\begin{equation}
\small
\begin{split}
\min \limits_{\theta_G} &\max \limits_{\theta_D}V(G,D)=\sum_{i=1}^{n}\sum_{j=1}^{n}(\mathbb{E}_{(v_i, v_j)\sim p_{\rm data}}[{\rm log}D(v_i,v_j;\theta_D)]\\
&+\mathbb{E}_{(v_i, v_a)\sim p_G}[{\rm log}(1-D(v_i,v_a;\theta_D))])
\end{split}
\label{ref:eqValue}
\end{equation}
where $(v_i,v_j)\sim p_{\rm data}$ denotes  the positive nodes pair and $(v_i,v_a) \sim p_G$ denotes an adversarial  sample obtained using the efficient sampling strategy outlined above.

% The Fig.(\ref{Fig_vis:framework}) illustrates the framework of the MVGAN. For the given two view networks, the orange vertices pair $(v_1 , v_2)$ represents the positive vertex pair sampled from $p_{data}$. For the given vertex $v_1$, we will input all the $(v_1, v_c)$ into the connectivity Generator where the blue nodes $v_c$ is selected from the adversarial set $\mathcal{C}$. After learning all the connectivity information, the connectivity generator $G$ would select the one vertex with the most similar connectivity ($v_4$ in the example) to fool the connectivity discriminator. The connectivity Generator $G$ is compose of $k$ view generators and one common generator $G_c$. The common generator $G_c$ generates the $2d$ dimensional representation of the input vertex pair and $k$ view generators which each generator $G^{(l)}$ takes $2d$ dimensional representation as input and output the connectivity $e_{ij}^{(l)}$ in $l$-th view. The parameter $\theta_D$ for the connectivity discriminator $D$ could be updated by SGD and the parameters $\theta_G = \{\theta_c, \theta^{(1)}, \dots, \theta^{(k)} \}$ of connectivity Generator $G$ could be updated under the policy gradient. We utilize the $\theta_c$ as the multi-view network embedding. [add reason]

% In the following subsections, we will fully discuss the sampling strategy, the connectivity Discriminator $D$, connectivity Generator $G$, and optimization for $D$ and $G$.

% \subsubsection*{Sampling strategy for multi-view networks}
% In multi-view graph scenario, one key question is how to draw positive
% and negative samples in the training phase efficiently. One kind of typical sampling strategies in graph representation learning is to collect random walks sequences via treating nodes as words from the language modelling perspective. In the multi-view graph cases, however, such strategy could not diffuse among views since there are no cross-view links. Another kind of typical sampling strategies is to sample the neighbors vertices randomly from its neighbors since the transit probability is equal to the connectivity distribution. Such method could not be directly extended to multi-view graph scenarios due the connectivity distribution could not be approximate by the transit probability.

% In the paper, we propose the sampling strategy to sample the positive vertices pair and its corresponding negative vertices pair from the multi-view network efficiently. During training process of MVGAN, we firstly sample the positive vertices pair $(v_i,v_j)$ over vertices set $\mathcal V$ randomly with the multi-view connectivity information $\mathcal{K}_{ij}$. Then for the given vertex $v_i$, we select $v_a$ from the $\mathcal V$ as:
% \begin{equation}
%     \argmin_{v_a \in \mathcal V}\prod_{l=1}^kp(e^{(l)}_{ij}|v_i,v_a)
%     \label{eq:select}
% \end{equation}

% The intuitive motivation behind the sampling strategy in Eq.(\ref{eq:select}) is that the negative vertices pair $(v_i, v_a)$ is more likely to fool the connectivity discriminator if connectivity $\tilde{\mathcal{K}}_{ia}$ approximates to the connectivity $\mathcal{K}_{ij}$ of the positive pair $(v_i, v_j)$. As the $D$ learns to distinguish the negative nodes from the positive nodes, the $G$ capture the connectivity distribution of the multi-view graph.

%\begin{equation}
%    \argmin_c \sum_{l=1}^k||e^{(l)}_{ic}-e^{(l)}_{ij}||_2, \quad \text{for}  \,\,\,  v_c \in  \bigcup\limits_{l=1}^{k} \mathcal{N}({v_i})
%\end{equation}
% However, directly searching for the $v_a$ in Eq.(\ref{eq:select}) is time-consuming. We obtain the best $v_c$ from  the subset $\mathcal C = \bigcup\limits_{l=1}^{k} \mathcal{N}({v_i})$.
%We use the Theorem.1 to show that we could obtain relatively good $v_c$ from the subset $\mathcal C = \bigcup\limits_{l=1}^{k} \mathcal{N}({v_i})$.

%\begin{theorem}
%In the multi-view network, if each view l follows the random graph $G(n, p^{(l)})$, for $\forall (v_i, v_j) \subset \mathcal{V} \times \mathcal{V}$, there exists the vertex $v_c \in \bigcup\limits_{l=1}^{k} \mathcal{N}({v_i})$ such that
%for the arbitrary vertices $v_i$ and $v_j$, there exists $v_c$ in the union set of the neighbors of $v_i$ such that $\mathcal{K}_{ij}$ approximate $\mathcal{K}_{ic}$. 
%\begin{equation*}
%p(||\mathcal{K}_{ij}-\mathcal{K}_{ic}||_1> \epsilon)\leq \frac{\sum n p(1-p)}{\epsilon^2}\\
%\end{equation*}
%\end{theorem}
%\begin{proof}
%Suppose the degree for vertex $v_i$ in view $l$ is  $\text{deg}^{(l)}(v_i)$.
%We firstly proof the theorem in two view case and then extend to $k$ views case. In the case of $\mathcal{K}_{ij}$ equals to $\{0,0\}, \{0,1\}, \{1,0\}$, it is obvious to we could find the $v_c$ in $\mathcal C$ such that $\mathcal{K}_{ic}=\mathcal{K}_{ij}$. 
%If $\mathcal{K}_{ij}=\{1,1\}$, the only case is that  $p(||\mathcal{K}_{ij}-\mathcal{K}_{ic}||_1> \epsilon) = \binom{n-dev^{(1)}(v)}{dev^{(2)}(v)-2}p^{dev^{(2)}(v)-2}(1-p)^{n-dev^{(1)}(v)}+\binom{n-dev^{(2)}(v)}{dev^{(1)}(v)-2}p^{dev^{(1)}(v)-2}(1-p)^{n-dev^{(2)}(v)}= Pr(k;n-dev^{(1)},p_2)+ Pr(k;n-dev^{(2)},p_1)$. In $k$ views case, we need to consider the situation  we could extend the framework to $k$ views as $Pr(k;n-dev^{(1)},p_2)+ Pr(k;n-dev^{(2)},p_1)$
%\end{proof}
% \subsubsection*{Connectivity Discriminator and  Generator}
% In this subsection, we introduce the novel connectivity Discriminator $D$ and connectivity Generator $G$. The connectivity discriminator $D$ should be able to differentiate the positive vertex pairs from the multi-view connectivity distribution and negative vertex pairs from the generator $G$ as accurately as possible. For arbitrary vertex pair $(v_i,v_j)$, $D$ should be the differentiable function such that $D(v_i,v_j)\rightarrow[0,1]$.
% %For any $(v_i, v_j)\simp_{data}$ and $(v_i, v_a)\simp_{g}$ 
% %\begin{equation}
% %    p(1|v_i,v_j)p(0|v_i,v_a)
% %\end{equation}
% %In other words, the discriminator $D(v_i, v_j; \theta_D)$ needs to discriminate the label $y_{ij}$ (either positive represented by $1$ or negative represented by $0$) for the given training vertex pair $(v_i,v_j)$. 
% In this case, we define the $D$ as the sigmoid function of the inner product of the input vertex pair $(v_i,v_j)$:
% \begin{equation}
%   D(v_i,v_j) =  \frac{\exp(d_i^T\cdot d_j)}{1+\exp(d_i^T\cdot d_j)}
%   \label{eq2:d}
% \end{equation}
% where $d_i$ and $d_j$ denote to the $k$ dimensional representation of vertex pair $(v_i,v_j)$. It worth note that $D(\cdot)$ could be any differentiable function with domain [0,1]. We choose the sigmoid function for simplification consideration. We leave this as a possible future direction. 

% The connectivity Generator $G$ aims to generate the adversarial vertex pairs that could fool the connectivity Discriminator $D$. For the given positive vertex $v_i$, the generator $G$ generate the all vertex pair $(v_i, v_c)$  to learn
% the connectivity 
% $\tilde{\mathcal{K}_{ic}} = (\tilde{e}_{ic}^{(1)}, \dots, \tilde{e}_{ic}^{(k)})$ over $\mathcal{C}$. More specifically, we model the 
% In MVGAN, we define the $G$ as:
% \begin{equation}
% \begin{split}
% \quad G(e^{(1)}_{ij},\dots,e^{(k)}_{ij}|v_i,v_j,\theta)= \prod_{l=1}^kG^{(l)}(e^{(l)}_{ij}|v_i,v_j,\theta_c,\theta^{(l)})
% \end{split}
% \label{eq4:g}
% \end{equation}
%In Eq.(\ref{eq:DisImp}), 
%$\theta = \{\theta_c, \theta^{(1)}, \dots, \theta^{(k)}\}$ 
% where $\theta_c$  is the common parameters share by all generators and $\theta^{(l)}$ is the specific parameters for the generator $G^{(l)}$. It worth note that the the k generators could be optimized simultaneously since they are independent. In the implementation, we use two layer MLP to implement each $G^{(l)}$ and $G_c$. Actually, more layers can be stacked and all the generators could be replaced by more sophisticated DNN. We leave this as a possible future direction. 


\subsection{Training Algorithm of MVNE-GAN}
Following the standard approach to  training GAN ~\cite{goodfellow2014generative,wang2018graphgan}, we alternate between the updates $D$ and $G$  with mini-batch gradient descent. \\
\vskip -0.8em
\noindent{}\textbf{Updating $D$:}
Given that $\theta_D = \{ d_i \}_{i=1}^n$ is differentiable w.r.t to the loss function in Eq.(\ref{ref:eqValue}), the gradient of $\theta_D$ is given as:
\begin{equation} 
\begin{split}
    &\nabla_{\theta_D}V(G,D) =\sum_{i=1}^{n}\sum_{j=1}^{n}(\mathbb{E}_{(v_i, v_j)\sim p_{\rm data}}[\nabla_{\theta_D}{\rm log}D(v_i,v_j)]\\
&+\mathbb{E}_{(v_i,v_c)\sim p_g}[\nabla \theta_D{\rm log}(1-D(v_i,v_c))])
\end{split}
\label{eq3:updateD}
\end{equation}
\vskip -0.5em
\noindent{}\textbf{Updating $G$:}
Since we sampled discrete data, i.e., the negative node IDs, from MVNE-GAN, the discrete outputs make it difficult to pass the gradient update from the discriminative model to the generative model. Following the previous work~\cite{wang2018graphgan}, we utilize the policy gradient to update the generator parameters $\theta_G = \{\theta_c, \theta^{(1)}, \dots, \theta^{(k)} \}$:
\begin{equation}
\begin{split}
    &\nabla_{\theta_G}V(G,D)\\ &=\nabla_{\theta_G} \sum_{i=1}^{n}\sum_{j=1}^{n}\mathbb{E}_{(v_i, v_c)\sim p_g}[{\rm log}(1-D(v_i,v_j)]\\
    &=\sum_{i=1}^{n}\sum_{j=1}^{n}\mathbb{E}_{(v_i, v_c)\sim p_g}[\nabla_{\theta_G}{\rm log}G(v_i,v_c){\rm log}(1-D(v_i,v_c))]
\end{split}
\label{eq3:updateG}
\end{equation}

\noindent{}\textbf{Training Algorithm}
With the update rules for $\theta_D$ and $\theta_G$ in place, the overall training algorithm is summarized in Algorithm \ref{Multi}. 
In Line 1, we initialize and pre-train the $D$ and $G$. From Line 3 to 6, we update parameters of $D$, i.e., $\theta_D$. From Line 7 to 9, we update the parameters of $G$, i.e., $\theta_G$. % During the training phase, the $D$ and $G$ are trained alternatively. 
The $D$ and $G$ play against each other until the MVNE-GAN converges.

\subsection{Theoretical Analysis} \label{sec:theorectical_analysis}
It has been shown in ~\cite{goodfellow2014generative} that $p_G$ could converge to $p_{data}$ in continuous space. In Proposition \ref{proposition}, we show that $p_G$ also converge $p_{data}$ in discrete space. In other words, upon convergence of Algorithm~\rf{Multi}, MVNE-GAN can learn embeddings that makes $p_g \approx p_{data}$, which captures the multi-view network topology. 
% . In the Proposition.2 shows the $p_g$ is converge to $p_{data}$ in Algorithm.(\ref{Multi}).

\begin{algorithm}
  \caption{\text{MVGAN} framework}
  \label{Multi}
  \begin{algorithmic}[1]
  \REQUIRE embedding dimension $d$, size of discriminating samples $t$, generating samples $s$
  % \ENSURE $G(\mathcal{K}_{ij}|v_i,v_j,\theta_G)$, $D(v_i,v_j,\theta_D)$
  \ENSURE $\theta_D$, $\theta_G$
 \STATE Initialize and pre-train $D$ and $G$  
  \WHILE{MVGAN not converged} 
%  \STATE  $ W_{appro}\gets H\Lambda H^T$
    \FOR {D-steps}
    \STATE  Sample $t$ positive nodes pairs $(v_i, v_i)$ from $p_{data}$ and $t$ negative
node pairs $(v_i, v_a)$ from $p_g$ for each node $v_i$
\STATE update $\theta_D$ according to Eq.(\ref{eq2:d}) and Eq.(\ref{eq3:updateD})
    \ENDFOR
   \FOR {G-steps}
    \STATE  Sample $s$ negative nodes pair $(v_i, v_a)$ for each node $v_i$
\STATE update $\theta_G$ according to Eq.(\ref{eq4:g}) and Eq.(\ref{eq3:updateG})
    \ENDFOR
  \ENDWHILE
  \end{algorithmic}
\end{algorithm}
%\noindent{}\textbf{Theoretical Analysis}  We use the lemma.2 to illustrate that $p_g$ is converge to $p_{data}$.
\begin{proposition}
\label{proposition}
If $G$ and $D$ have enough capacity, the discriminator is allowed to reach its optimum given $G$, and $p_g$ is converge to $p_{data}$
\end{proposition}
\begin{proof}
Consider $V (G, D) = U(p_g, D)$ as a function of $p_g$. Note that $U(p_g, D)$ is convex in $p_g$. The subderivatives of a supremum of convex functions include the derivative of the function at the point where the maximum is attained.
This is equivalent to computing a gradient descent update for $p_g$ at the optimal $D$ given the corresponding
G. 
%supD U(pg, D) is convex in pg with a unique global optima 
Therefore with sufficiently small updates of $p_g$, $p_g$ converges to $p_{data}$, concluding the proof.
\end{proof}

==> model.tex <==
\section{Multi-View Network Embedding GAN}
In what follows, we define multi-view network embedding problem before describing the key components of MEGAN, our proposed solution to multi-view network embedding.
\subsection{Multi-View Network Embedding}
A multi-view network is defined as $\mathcal{G} = (\mathcal{V} ,\mathcal{E})$, where $\mathcal{V}= \{v_1, v_2, \dots, v_n \}$ denotes the set of nodes and $\mathcal{E}=\{\mathcal{E}^{(1)},\mathcal{E}^{(2)}, \dots, \mathcal{E}^{(k)}\} $ describes the edge sets that encode  $k$ different relation types (views).
For a given relation type $l$, $\mathcal{E}^{(l)} = \{e_{ij}^{(l)}\}_{i,j=1}^n$ specifies the presence of the corresponding relation between node $v_i$ and node $v_j$. Thus, $e_{ij}^{(l)}=1$ indicates that $v_i$ and $v_j$ has a link for relation $l$ and 0 otherwise.  We use $\mathcal{K}_{ij} = (e_{ij}^{(1)}, \dots, e_{ij}^{(k)})$ to denote the connectivity of $(v_i,v_j)$ in multi-view topology. The goal of multi-view network representation learning is to learn $\mathbf{X} \in \mathbb{R}^{n \times d}$, a low-dimensional embedding of $\mathcal{G}$, where $d \ll n$ is the latent dimension.
\begin{figure}[ht!]
      \centering
   %   \vskip -1em
        \includegraphics[width=9cm]{archframe.eps}
  %      \vskip -0.3em
        \caption{The architecture of MEGAN framework. The pair of the orange nodes $(v_1,v_2)$  denotes {\em real} pair of nodes. For each blue nodes $v_c$, the generator learns its connectivity $\{e^{(1)}_{ic},e^{(2)}_{ic}\}$ and generates {\em fake} pair of nodes which could fool the discriminator with highest probability. In the example, $(v_1, v_4)$ is selected to fool the discriminator.}
        \label{fig:model_architecture}
        \vskip -1em
\end{figure}
%type of each relation $e^{(l)} = \{ e_{ij}^{(l)}\}_{i,j=1}^{|l|}$, . 

%between node set $\Phi^{(k)} (\mathcal{V})$. For type of each relation $e^{(l)} = \{ e_{ij}^{(l)}\}_{i,j=1}^{|l|}$, 

%Figure~\ref{fig:model_architecture} illustrates the architecture of MEGAN.
\subsection{\textbf{Multi-view Generative Adversarial Network}}
Unlike a GAN designed to perform single-view network embedding, which needs to model only the connectivity among nodes within a single view, the MEGAN needs to capture the connectivity among nodes within each view as well as the correlations between views. To achieve this, given the \textit{real} pair of nodes $(v_i, v_j) \sim p_{data}$, MEGAN consists of two modules: a \textbf{generator} which generates (or chooses) a \textit{fake} node $v_c$ with the connectivity pattern $\mathcal K_{ic}$ between $v_i$ and $v_c$ being sufficiently similar to that of the real pair of node; and a \textbf{discriminator} which is trained to distinguish between the real pair of nodes $(v_i,v_j)$ and \textit{fake} pair of node $(v_i,v_c)$.
Figure~\ref{fig:model_architecture} illustrates the architecture of MEGAN. For the pair of nodes $(v_1, v_2)$, the generator produces a \textit{fake} node $v_4$ forming the pair of nodes $(v_1, v_4)$ to fool the discriminator and  the discriminator is trained to differentiate if a pair of nodes input to it is \textit{real} or \textit{fake}. With the minmax game between $D$ and $G$, we will show that upon convergence, we are able to learn embeddings that $G$ can use to generate the multi-view network. In such situation, the learned embeddings is able to capture the connectivity among nodes within each views and the correlations between views. Next, we introduce the details of $G$, $D$ and an efficient sampling strategy.

\subsubsection{Multi-view Generator}
Recall that goals of multi-view generator $G$ are to \textbf{(i)} generate the multi-view connectivity of fake nodes that
fools the discriminator $D$; and \textbf{(ii)} learn an embedding  that captures the multi-view network topology. To ensure that it achieves the goals, we design the multi-view generator consisting of two components: one fusing generator $G_f$ and $k$ connectivity generators $G^{(l)}$. Let $\mathbf{X} \in \mathbb{R}^{n \times d}$ be the network embedding matrix we want to learn, then the representation of $v_i$ can be obtained as $\mathbf{e}_i^T \mathbf{X}$, where $\mathbf{e}_i$ is the one-hot representation with $i$-th value as 1. The fusing generator $G_f$ firstly fuses the representation of $v_i$ and $v_j$, aiming to capture the correlation between $v_i$ and $v_j$.  We use $G_f(v_i, v_j; \mathbf{X}, \theta_f)$ to denote the fused representation where $\theta_f$ is its parameters. Then, the fused representation is used to calculate the probability of $e_{ij}^{(l)}=1$ for $l=1,\dots, k$. This can be formally written as:
\begin{equation}
\small
\begin{split}
G(e^{(1)}_{ij},\dots,e^{(k)}_{ij}|v_i,v_j,\theta_G)= \prod_{l=1}^kG^{(l)}(e^{(l)}_{ij}|G_f(v_i,v_j;\mathbf{X},\theta_f);\theta^{(l)})
\end{split}
\label{eq4:g}
\end{equation}
%In Eq.(\ref{eq:DisImp}), 
%$\theta = \{\theta_c, \theta^{(1)}, \dots, \theta^{(k)}\}$ 
where $G^{(l)}$ is the connectivity generator for generating the connectivity in between $(v_i,v_j)$ in view $l$ given the fused representation and $\theta^{(l)}$ is the parameter for $G^{(l)}$. $\theta_G=\{\mathbf{X}, \theta_f, \theta^{(l), l =1, \dots, k}\}$ is the parameter for the multi-view generator $G$. Because each $G^{(l)}$ of $k$ generators are independent given the fused representation, the corresponding parameter $\theta^{(l)}$ can be optimized independently in parallel. We use two layer multi-layer perceptron (MLP) to implement $G_f$ and each $G^{(l)}$. Actually, more complex deep neural networks could replace the generative model outlined here. We leave exploring feasible deep neural networks as a possible future direction. To fool the discriminator, for each $(v_i,v_j) \sim p_{data}$, where $p_{data}$ represents the multi-view connectivity, we propose to sample a pair of negative nodes from $G$ that has connectivity that is similar to that of  $(v_i, v_j)$, e.g., $(v_i, v_c) \sim p_g$ with $\tilde{\mathcal{K}}_{ic}=\mathcal{K}_{ij}$, where $p_g$ denotes the distribution modeled by $G$. In particular, we choose the $v_c$ that has the highest probability as:
\begin{equation}
\argmax_{v_c \in \mathcal V}\prod_{l=1}^k G^{(l)}(e^{(l)}_{ic} =e^{(l)}_{ij} |v_i,v_j,G_f(v_i,v_j;\mathbf{X},\theta_f)
    \label{eq:select}
\end{equation}
The motivation behind the negative sampling strategy in Eq.(\ref{eq:select}) is that the negative node pair $(v_i, v_c)$ is more likely to fool the connectivity discriminator if connectivity $\tilde{\mathcal{K}}_{ic}$ is the same to the connectivity $\mathcal{K}_{ij}$ of the positive pair $(v_i, v_j)$. \textit{The objective of $G$ is then to update network embedding $\mathbf{X}$ and $\theta_G$ so that the generator has higher chance of producing negative samples that can fool the discriminator $D$}.

\subsubsection{Node Pair Discriminator}
The goal of $D$ is to discriminate between the positive node pairs from the multi-view network data and the negative node pairs produced by the generator $G$ so as to enforce $G$ to more accurately fit the distribution of multi-view network connectivity. For this purpose, for an arbitrary node pair sampled from real-data, i.e., $(v_i,v_j) \sim p_{data}$, $D$ should output 1, meaning that the sampled node pair is real. 
% The reason we want to select the node $v_j$ that has the highest probability of having $\mathcal{K}_{jc}=\mathcal{K}_{ic}$ is because we want to fool the discriminator. The one that has the highest probability of having the same connectivity is more likely to fool the discriminator. 
Given such a negative or fake edge (pair of nodes), the discriminator should output 0, whereas $G$ should aim to assign high enough probability to negative pair of nodes that can fool $D$. 
As $D$ learns to distinguish the negative pair of nodes from the positive ones, the $G$ captures the connectivity distribution of the multi-view graph. 
%With such minmax game, for a given pair of nodes $(v_i, v_c)$, when we want to sample $(v_j, v_c)$ with $\tilde{\mathcal{K}}_{ic}=\mathcal{K}_{jc}$, we can expect the generator will gradually assign higher probability to $(v_i, v_c)$ because this is the one that can finally fool the discriminator upon convergence. 
We will show this in Section~\ref{sec:theorectical_analysis}.
%For any $(v_i, v_j)\simp_{data}$ and $(v_i, v_a)\simp_{g}$ 
%\begin{equation}
%    p(1|v_i,v_j)p(0|v_i,v_a)
%\end{equation}
%In other words, the discriminator $D(v_i, v_j; \theta_D)$ needs to discriminate the label $y_{ij}$ (either positive represented by $1$ or negative represented by $0$) for the given training vertex pair $(v_i,v_j)$. 

We define the $D$ as the sigmoid function of the inner product of the input node pair $(v_i,v_j)$:
\begin{equation}
\small
   D(v_i,v_j) =  \frac{\exp(\mathbf{d_i}^T\cdot \mathbf{d_j})}{1+\exp(\mathbf{d_i}^T\cdot \mathbf{d_j})}
   \label{eq2:d}
\end{equation}
where $\mathbf{d}_i$ and $\mathbf{d}_j$ denote the $d$ dimensional representation of node pair $(v_i,v_j)$. It is worth noting that $D(v_i,v_j)$ could be any differentiable function with domain $[0,1]$. We choose the sigmoid function for its stable property and leave the selections of $D(\cdot)$ as a possible future direction.

\subsubsection{Efficient Negative Node Sampling}
In practice, for one pair of nodes $(v_i,v_j)$, in order to sample a pair of nodes $(v_i, v_c)$ from $G$, we need to calculate Eq.(\ref{eq:select}) for all $v_c \in \mathcal{V}$ and select the $v_c$ with the highest probability, which can be very time-consuming. To make the negative sampling more efficient, instead of calculating the probability for all nodes, we  calculate the probability  for neighbors of $v_i$, i.e., $\mathcal{N}(v_i)$, where $\mathcal{N}(v_i)$ is the set of nodes that have connectivity to $v_i$ for at least one view in real network. In other words, we only sample from $\mathcal{N}(v_i)$. The size of $\mathcal{N}(v_i)$ is significantly smaller than $n$ because the network is usually very sparse, which makes the sampling very efficient. %Thus, we would expect that for positive sample $(v_i,v_j) \sim p_{data}$, any negative sample $(v_i,v_c)$ should have a node $v_c$ from $v_i$'s neighbor.  


%{\color{blue} to revise} In multi-view graph scenario, one key question is how to draw positive and negative samples in the training phase efficiently. One kind of typical sampling strategies in graph representation learning is to collect random walks sequences via treating nodes as words from the language modelling perspective. In the multi-view graph cases, however, such strategy could not diffuse among views since there are no cross-view links. Another kind of typical sampling strategies is to sample the neighbors vertices randomly from its neighbors since the transit probability is equal to the connectivity distribution. Such method could not be directly extended to multi-view graph scenarios due the connectivity distribution could not be approximate by the transit probability.

% In the paper, we propose the sampling strategy to sample the positive vertices pair and its corresponding negative vertices pair from the multi-view network efficiently. During training process of MVGAN, we firstly sample the positive vertices pair $(v_i,v_j)$ over vertices set $\mathcal V$ randomly with the multi-view connectivity information $\mathcal{K}_{ij}$. Then for the given vertex $v_i$, we select $v_a$ from the $\mathcal V$ as:
% \begin{equation}
%     \argmin_{v_a \in \mathcal V}\prod_{l=1}^kp(e^{(l)}_{ij}|v_i,v_a)
%     \label{eq:select}
% \end{equation}




\subsubsection{Objective Function of MEGAN}

% In multi-view network, we assume that the connectivity information $\mathcal{K}_{ij} = (e_{ij}^{(1)}, \dots, e_{ij}^{(k)})$ of the vertex pair $(v_i,v_j)$ reveals the connectivity distribution $p_{data}(\mathcal{K}_{ij}|v_i,v_j)$. %among $k$ types of relations. 
% In the MVGAN model, we propose a connectivity generator $G$ which tries to capture the connectivity distribution  $p_{data}(\mathcal{K}_{ij}|v_i,v_j)$ of pair $(v_i,v_j)$ and generate the negative vertex pair $(v_i,v_a)$ to fool the connectivity discriminator $D$. Meanwhile, we train the connectivity discriminator $D$ which learns to distinguish the positive vertices pair sampled from $p_{data}(\mathcal{K}_{ij}|v_i,v_j)$ and the adversarial vertices sampled from $p_g(\tilde{\mathcal{K}}_{ia}|v_i,v_a)$. The joint value function $V(G,D)$ could be define as:
With generator modeling multi-view connectivity to generate fake samples that could fool the discriminator, discriminator differentiates between true pairs of nodes from fake pairs of nodes. We specify the objective function for MEGAN: 
\begin{equation}
\small
\begin{split}
\min \limits_{\theta_G} &\max \limits_{\theta_D}V(G,D)=\sum_{i=1}^{n}(\mathbb{E}_{(v_i, v_j)\sim p_{\rm data}}[{\rm log}D(v_i,v_j;\theta_D)]\\
&+\mathbb{E}_{{(v_i,v_c)\sim p_g}}[{\rm log}(1-D(v_i,v_c;\theta_D))])
\end{split}
\label{ref:eqValue}
\end{equation}
where $(v_i,v_j)\sim p_{\rm data}$ denotes the positive nodes pair and $(v_i,v_c) \sim p_g$ denotes the fake pair of nodes obtained using the efficient negative sampling strategy outlined above. \textit{Through such minmax game, we can learn network embedding $\mathbf{X}$ and the generator $G$ that can approximate the multi-view network to fool the discriminator}. In other words, the learned network embedding $\mathbf{X}$ is able to capture the connectivity among nodes within each views and the correlations between views.

\subsection{Training Algorithm of MEGAN}
Following the standard approach to  training GAN ~\cite{goodfellow2014generative,wang2018graphgan}, we alternate between the updates $D$ and $G$  with mini-batch gradient descent. \\
%\vskip -0.8em
\noindent{}\textbf{Updating $D$:}
Given that $\theta_D = \{ d_i \}_{i=1}^n$ is differentiable w.r.t to the loss function in Eq.(\ref{ref:eqValue}), the gradient of $\theta_D$ is given as:
\begin{equation}
\small
\begin{split}
    &\nabla_{\theta_D}V(G,D) =\sum_{i=1}^{n}(\mathbb{E}_{(v_i, v_j)\sim p_{\rm data}}[\nabla_{\theta_D}{\rm log}D(v_i,v_j)]\\
&+\mathbb{E}_{{(v_i,v_c)\sim p_g}}[\nabla \theta_D{\rm log}(1-D(v_i,v_c))])
\end{split}
\label{eq3:updateD}
\end{equation}
%\vskip -0.5em
\noindent{}\textbf{Updating $G$:}
Since we sampled discrete data, i.e., the negative node IDs, from MEGAN, the discrete outputs make it difficult to pass the gradient update from the discriminative model to the generative model. Following the previous work~\cite{yu2017seqgan,wang2018graphgan}, we utilize the policy gradient to update the generator parameters $\theta_G = \{\mathbf{X}, \theta_f, \theta^{(1)}, \dots, \theta^{(k)} \}$:
\begin{equation}
\small
\begin{split}
    &\nabla_{\theta_G}V(G,D)\\ &=\nabla_{\theta_G} \sum_{i=1}^{n}\mathbb{E}_{(v_i,v_c)\sim p_g}[{\rm log}(1-D(v_i,v_c;\theta_D)]\\
     &=\nabla_{\theta_G}\sum_{i=1}^{n}\sum_{c=1}^{n} G(\mathcal K_{ic}|v_i,v_c)[{\rm log}(1-D(v_i,v_c;\theta_D)]\\
        &=\sum_{i=1}^{n}\mathbb{E}_{(v_i,v_c)\sim G}[\nabla_{\theta_G}{\rm log}G(\mathcal K_{ic}|v_i,v_c){\rm log}(1-D(v_i,v_c;\theta_D))]
\end{split}
\label{eq3:updateG}
\end{equation}

\noindent{}\textbf{Training Algorithm}
With the update rules for $\theta_D$ and $\theta_G$ in place, the overall training algorithm is summarized in Algorithm \ref{Multi}. 
In Line 1, we initialize and pre-train the $D$ and $G$. From Line 3 to 6, we update parameters of $G$, i.e., $\theta_G$. From Line 7 to 10, we update the parameters of $D$, i.e., $\theta_D$ % During the training phase, the $D$ and $G$ are trained alternatively. 
The $D$ and $G$ play against each other until the MEGAN converges.

\subsection{Theoretical Analysis} \label{sec:theorectical_analysis}
It has been shown in ~\cite{goodfellow2014generative} that $p_g$ could converge to $p_{data}$ in continuous space. In Proposition \ref{prop:1}, we show that $p_g$ also converge $p_{data}$ in discrete space. In other words, upon convergence of Algorithm~\ref{Multi}, MEGAN can learn embeddings that makes $p_g \approx p_{data}$, which captures the multi-view network topology. 
% . In the Proposition.2 shows the $p_g$ is converge to $p_{data}$ in Algorithm.(\ref{Multi}).

\begin{algorithm}[t]
  \caption{\text{MVGAN} framework}
  \label{Multi}
  \begin{algorithmic}[1]
  \REQUIRE embedding dimension $d$, size of discriminating samples $t$, generating samples $s$
  % \ENSURE $G(\mathcal{K}_{ij}|v_i,v_j,\theta_G)$, $D(v_i,v_j,\theta_D)$
  \ENSURE $\theta_D$, $\theta_G$
 \STATE Initialize and pre-train $D$ and $G$  
  \WHILE{MVGAN not converged} 
%  \STATE  $ W_{appro}\gets H\Lambda H^T$
  \FOR {G-steps}
    \STATE  Sample $s$ negative pairs of nodes $(v_i, v_c)$ for the given   positive pair of nodes $(v_i,v_j)$
\STATE update $\theta_G$ according to Eq.(\ref{eq4:g}) and Eq.(\ref{eq3:updateG})
    \ENDFOR
    \FOR {D-steps}
    \STATE  Sample $t$ positive nodes pairs $(v_i, v_j)$ and $t$ negative
node pairs $(v_i, v_c)$ from $p_g$ for each node $v_i$
\STATE update $\theta_D$ according to Eq.(\ref{eq2:d}) and Eq.(\ref{eq3:updateD})
    \ENDFOR
  \ENDWHILE
  \end{algorithmic}
\end{algorithm}
%\noindent{}\textbf{Theoretical Analysis}  We use the lemma.2 to illustrate that $p_g$ is converge to $p_{data}$.
\vskip -1.1em
\begin{proposition}
%[Propositions]
\label{prop:1}
If $G$ and $D$ have enough capacity, the discriminator and the generator are allowed to reach its optimum, and $p_g$ is converge to $p_{data}$ based on the update rule in Algorithm \ref{Multi}.
\end{proposition}
\begin{proof}
The proof is similar to ~\cite{goodfellow2014generative}, and we omit the details here.
\end{proof}
\vskip -1.1em

